Hybrid Quantum-Classical Eigensolver Without Variation or Parametric Gates

The use of near-term quantum devices that lack quantum error correction, for addressing quantum chemistry and physics problems, requires hybrid quantum-classical algorithms and techniques. Here we present a process for obtaining the eigenenergy spectrum of electronic quantum systems. This is achieved by projecting the Hamiltonian of a quantum system onto a limited effective Hilbert space specified by a set of computational bases. From this projection an effective Hamiltonian is obtained. Furthermore, a process for preparing short depth quantum circuits to measure the corresponding diagonal and off-diagonal terms of the effective Hamiltonian is given, whereby quantum entanglement and ancilla qubits are used. The effective Hamiltonian is then diagonalized on a classical computer using numerical algorithms to obtain the eigenvalues. The use case of this approach is demonstrated for ground sate and excited states of BeH$_2$ and LiH molecules, and the density of states, which agrees well with exact solutions. Additionally, hardware demonstration is presented using IBM quantum devices for H$_2$ molecule.

==> Archive/UCCandVQA.tex <==
%  This is a revew of the UCC ansatz and VQA approach

% \subsection{Ground state ansatz}
% \label{sec-ucc}



% Let us now consider a purterbative approach where the series in Eq. (\ref{eq-ansatz-ucc}) is cut off at some order; for example only the S and D types are retained in the series. The ground state can then be written as 
% \begin{eqnarray}
% \ket{ \psi} &=& \sum_{\bf{n}} c_{\bf{n}} \ket{\bf{n}},
% \label{eq-ansatz-1}
% \end{eqnarray}
% with only a polynomial number of Fock bases $\{\ket{\bf{n}}\}$. Let us denote this number by $N^\alpha$ for some fixed $\alpha$ value. For example the situation where only D types are considered in Eq. (\ref{eq-ansatz-ucc}), $N^\alpha = {{N_f}\choose{2}} {{N-N_f}\choose{2}} < \mathcal{O}(N^4)$

% Now, suppose a quantum algorithm is designed that evaluates the matrix elements 
% $\bra{\bf n^\prime} \hat{H} \ket{\bf n}$. Then, effective Hamiltonian 
% \begin{eqnarray}
% \hat{H}_{eff} = 
% \begin{bmatrix} 
% \bra{\bf 0} \hat{H} \ket{\bf 0} 
% & \cdots 
%  & 
%  \\ 
% \vdots &
% \ddots &
% \vdots \\
% \, 
% & 
% \dots        
%  & \bra{\bf N^\alpha} \hat{H} \ket{\bf N^\alpha} \\
% \end{bmatrix}
% \quad
% \label{eq-H-eff}
% \end{eqnarray}
% can be diagonalized on a classical computer. The ground state of this effective Hamiltonian is an approximation to the ground state of the problem. In addition it provides a complete $N^\alpha$ orthogonal eigen states that approximate the low-lying exciations of the original problem.


% We should emphasize that the UCC ansatz is certainly richer than the approximation we considered here, as it is an infinite series compacted in the form of a unitary operation. However, in practice the implementation always require trotterization and many other approximation that impedes the purpose in practice. More importantly,  UCC is technique for the calculation of the ground state on a quantum computer. The quantum computation of the  excitated states using VQAs is computationally much more complex  (excited states).

% In contrast to to VQAs, either by using UCC ansatz or other heuristic ones, our approach is not variational. The matrix elements ain Eq. () are calculated by specific rotation of some $\alpha \log{(N)} $ ancillary qubits as explained in the next section.





% The unknown amplitudes $\{c_{i \nu}\}$, $\{c_{ij\nu\beta}\}$, etc. in Eq. (\ref{eq-ansatz-ucc}) can be specified through different approaches, and one of these approaches is variational principle; That is the values are varied until the minimum $\bra{\psi}\hat{H}\ket{\psi}$ is achieved. This variational approach has lead to the active area of Variational Quantum Algorithms for finding the ground state of small molecular compounds.

% Execution of VQAs using quantum processors is done applying a series of parametric gates on a set of initialized qubits that represent the reference frame $\ket{\bf 0}$. The outcome of the execution of the quantum circuit is a quantum state that approximates as much as possible an ansatz in the form of Eq. (\ref{eq-ansatz-ucc}). This parametric wave function is used to measure the Hamiltonian and estimate the energy. The execution is then repeated many times and by the use of classical optimizers the best parameters and ansatz that minimizes the Hamiltonian is found.

% However, in almost all the VQAs the relation between the parameters in the parametric gates and the variable amplitudes in Eq. (\ref{eq-ansatz-ucc}) is not trivial. In general, it is not clear what the amplitudes are, given a set of parametrs for the  gates. In addition, the design of the quantum circuit is always with the consideration of depth f the circuit and available gates at the hardware level. In most cases the quantum circuits can be non-intuitive, and practically hard to trace the transformation of the reference state $\ket{\bf 0}$ to the ansatz in Eq. (\ref{eq-ansatz-ucc}) is almost lost.


%  These states are chosen to be the first few excitations above a reference state as in Eq. (\ref{eq-ansatz-ucc}), and thus are polynomial in $N$.


% number of these elements are polynomial in $N$ since we

% The corresponding matrix, the effective Hamiltonian, is then diagonialized on a classical computer. Upon the digonalization, not only the amplitudes $c_{i,\nu}, \dots$ of the ground state but a polynomial number of orthogonal basis set is obtained as well. This set approximates some of the low-lying excited states of the many-problem. 

% Since we only retain a polynomial number $\{ \ket{\bf n} \}$, $N^\alpha$ for some fixed $\alpha$, the effective Hamiltonian matrix is $N^\alpha \times N^\alpha$; feasible to be diagonalized on classical computers.

% The challenge in this approach is to obtain the off-diagonal matrix elements. In the next section we show this can be done by an overhead ancillary qubits. the required number is at most logarithmic in $N$.  The approach requires both pre-processing and post-processing of the measured values on a classical computer, thus a hybrid quantum classical approach.

==> Archive/bibitems.tex <==


\cite{RevModPhys.83.1057}

==> Archive/grouping_chemistry.tex <==
\subsection{Quantum Chemistry Problems}

\subsubsection{Background}

For most practical quantum chemistry problems that are 
the main focus of recent quantum computers, the Hamiltonian can be expressed as
\begin{eqnarray}
\hat{H}  =
%%%
\sum_{ij} t_{ij} \,\,
a^{\dagger}_i \,   a_j +
%%
\sum_{ijkl} v_{ijkl} \,\,
a^{\dagger}_i \,  a^{\dagger}_j \,     a_k \,     a_l.
%%%%
\label{eq-generic-SQ-H-1}
\end{eqnarray}
A common task performed using HQC set-up is the evaluation of the ground state energy of this Hamiltonian. In the following we briefly review
the steps involved in this task before introducing a way to group the terms.

%% The Hamiltonian- coefficients
In the Hamiltonian above matrix elements $t_{ij}$ and $v_{ijkl}$ are calculated by a classical computer. In practice a software is used to evaluate these matrix elements, which are usually the matrix elements of the kinetic and Coulomb potential operators with respect to a single-electron spin-orbital basis set. 

%% The Hamiltonian- coefficients
%%%%%%%%
In practice the Hamiltonian in Eq. (\ref{eq-generic-SQ-H-1}) is stored as a list of tuples of coefficients and the corresponding products of creation and annihilation operators. In Eq. (\ref{eq-generic-SQ-H-1}), 
the terms of the first sum  are stored in a set $\{ (t_{ij}, a^\dagger_i a_j) \}$, and of the second sum in a set $\{ (v_{ijkl}, a^\dagger_i a^\dagger_j a_k a_l ) \}$.
This notation is a more convenient way to represents the input information of a given Hamiltonian.

The number of the elements in the set can further be reduced by normal ordering. In our notation, the normal ordering can be shown as
$$:(v_{ijkl},\,\, a^\dagger_i a^\dagger_j a_k a_l): \,\,\, =  (v^\prime_{ijkl},\,\, a^\dagger_i a^\dagger_j a_k a_l).$$
Here $:\,\, :$ stands for 
\normalem
\emph{
normal ordering.}
\ULforem 
If a sign factor  arises from the rearrangement, it is included in the coefficient ($v^\prime_{ijkl}$).
%%%%%%%%

On the quantum processor a qubit represents a spin-orbital level; The state of the qubit $\ket{0}$ ($\ket{1}$) represents an occupied (unoccupied) spin-orbital level. These qubits are labeled linearly from $1$ to $n$. Thus, it is better to rearrange the place of creation and annihilation operators in a normal ordered term so that the arrangement of the indices matches the enumeration of the qubits on the quantum device. For this purpose, it is useful to introduce an
\normalem
\emph{index ordering}
\ULforem
operation on a normal ordered term as in 
\begin{eqnarray}
\mathcal{I} \left[
:(
v_{ijkl}, \,\, 
a^\dagger_i a^\dagger_j a_k a_l
): 
\right]  &=& \,\,
\mathcal{I} \left[
(
v^{\prime}_{ijkl}, \,\, 
a^\dagger_i a^\dagger_j a_k a_l
) \right]
\nonumber \\
&=& \,\,
(
v^{\prime\prime}_{ijkl}, \,\, 
a^\dagger_{i} a_{k} a^\dagger_{j} a_{l}
).
\end{eqnarray}
Here operators are sorted such that their indices are arranged as $i\le k \cdots$; however, no index can appear more than twice, since that infers creation (or annihilation) of more than one fermion at a single spin-orbital level.  If two indices are equal, we make the convention that the creation is placed to the left of the annihilation.
Since in a normal ordered product the creation operators are to the right of annihilation operators, it is straightforward to verify that moving operators does not create additional terms.  Therefore, a normal ordered term is equal to its index-ordered up to a sign factor that is stored in a re-adjusted corresponding coefficient; For example $v_{ijkl}^{\prime \prime}= \xi\, \, v_{ijkl}^{\prime} $ if $\xi$ is the sign factor as a result of rearranging operators. 



All the steps above, that is the storage of the  coefficients and corresponding terms, algebraic manipulation, ordering and reduction of terms, is done on a classical computer using softwares designed for this purpose. A software package that performs these type of tasks is
for example Openfermion. 


The last step in preparing the terms in a Hamiltonian for measurement is mapping the  annihilation and creation operators onto 
Pauli matrices. This step is also performed on a classical computer, and a software such as
Openfermion is used in doing so as well.


Second quantized terms are transformed onto Pauli matrices by a map such as Jordan Wigner. Jordan Wigner (JW) transformations are defined as
%%%%%%%%%%%%%
\begin{eqnarray}
a_j^\dagger  &=&
%%%
\frac{1}{2} \left(\prod_{k}^{j-1} \hat{Z}_k \right )\,\,
(\hat{X}_j + i \hat{Y}_j)
\label{eq-JW-1}
\end{eqnarray}
and
\begin{eqnarray}
a_j  &=&
%%%
\frac{1}{2}  \left(\prod_{k}^{j-1} \hat{Z}_k \right)\,\,
(\hat{X}_j - i \hat{Y}_j).
\label{eq-JW-2}
\end{eqnarray}
JW maps creation  and annihilation operators onto the Pauli strings while keeping the relations in Eq (\ref{eq-sq-rel}) invariant \footnote{The Klein factor is dropped out since it changes the weight and not the Pauli String itself; Thus, not changing the results provided in this section.}. Performing the JW on the indexed ordered set of terms (on a classical computer), the output is a set of Pauli strings and corresponding  weights. 
The quantum processor is then instructed to measure this set of 
Pauli strings. 

In current approach to the measurement of the Pauli strings, each string is measured separately. If the number of the 
Pauli strings in the set is $n_h$, 
at most $n_h$ number of measurement is required to specify the expectation value of the the given Hamiltonian. In practice, in order to measure a Pauli string within a given accuracy $\epsilon$ the quantum circuit must be run $\mathcal{\frac{1}{\epsilon^2}}$. Therefore,  grouping the Pauli strings, yields to a significant speed-up. 

In order to use the measurement circuit introduce in  Sec. \ref{sec-q-circ} when a Hamiltonian of the form of Eq. (\ref{eq-generic-SQ-H-1}) is given, we need to show that grouping the terms into $n_g$ sets is possible, that provides a speed-up of $\mathcal{O}(n_h/n_g)$. For that purpose, we first categorize the types of Pauli strings that emerges from the JW transformation. 

In the following we investigate different category of Pauli strings that arise from JW transformation of the terms in Hamiltonian Eq. (\ref{eq-generic-SQ-H-1}) when provided as an indexed ordered set. To illustrate the grouping strategy we are seeking after, it is perhaps easier to begin with
$\{ (t_{ij}, a^\dagger_i a_j) \}$. A term $a^\dagger_i a_j$ is already normal ordered. A further index ordering, followed by JW, yields to two types of Pauli strings. First case is when $i  = j$:
\begin{eqnarray}
\{ \mathcal{I}\left[ (t_{ii},\,\, a^\dagger_i a_i ) \right]\}  &\rightarrow&
\{ 
\hat{n}_i = \frac{(\hat{I}_i+\hat{Z}_i)}{2}
\} \nonumber \\
&=& S_0.
\end{eqnarray}
The second case is when $i \ne j$:
\begin{eqnarray}
\{ \mathcal{I}\left[ (t_{ij},\,\, a^\dagger_i a_j ) \right]\}  &\rightarrow&
\{ 
\hat{O}_{i_1}
-
\hat{O}_{i_2} 
\vert \,\,
i_1<i_2, \,\,
\hat{O} \in \{\hat{X}, \hat{Y} \}
\}. \nonumber \\
\end{eqnarray}
where 
\begin{eqnarray}
\hat{O}_{i} 
-
\hat{O}_{j}
&=& 
\hat{O}_{i} 
\otimes
\left( \bigotimes_{k=i+1}^{k=j-1}\hat{Z}_k \right)
\otimes
\hat{O}_{j}.
\end{eqnarray}

Since Pauli strings in $S_0$ are all commuting and composed of only $Z$-Pauli matrices, the measurement of this set can be done simultaneously. 

In the second case where $i \ne j$ there are $\binom{n}{2}$ different strings for fixed $\hat{O}_{i_1}$ and $\hat{O}_{i_2}$. Since there two choices for these two operators, the total number of strings is $2^4 \binom{n}{2}$. However, following the two steps outlined in the previous section it is easy to identify the following four sets $S_{i_1; XX}$, $S_{i_1; YX}$, $S_{i_1; XY}$, and $S_{i_1; YY}$, where $S_{i_1; OQ}$ is
\begin{eqnarray}
S_{i_1; O,Q}  &=&
\{ 
\hat{O}_{i_1}
-
\hat{Q}_{i_2} 
\vert \,\, \forall i_2: 
i_1<i_2 \}
\}.
\end{eqnarray}
All the elements in a set $S_{i_1; O, Q}$ muttually anti-commute. Further, considering 
$S_{i_1; X,X}$ to be equivalent of $S_g$ in Eq. (\ref{eq-set}), a subset of $S_{i_1; Y,Y}$,  $A_g$, can always be chosen such that $M_g = S_g \cup A_g$ has $\vert M_g \vert = 2^m-1$ for an integer $m$. This is true because the number of elements in subsets of   $S_{i_1; Y,Y}$ range from $1$ to $\vert S_{i_1; X,X} \vert$. Therefore, if  $2^{m-1}-1 < \vert S_{i_1; X,X} \vert < 2^m -1$, we can always find the subset $A_g$ to satisfy the  $\vert M_g \vert = 2^m-1$. 

The same argument applies to all of the four sets $S_{i_1; XX}$, $S_{i_1; YX}$, $S_{i_1; XY}$, and $S_{i_1; YY}$. The number of $S_{i_1; OQ}$ sets for different is  $n_g = \mathcal(O)(2^2n)$, since there are $n-1$ way to choose $i_1$ and $4$ choices for $O$ and $Q$ indices. 
Thus, in order to measure the complete set of $\{ (t_{ij}, a^\dagger_i a_j) \}$, with $n_h = \mathcal{O}((2n)^2) $, using the quantum circuit Sec. \ref{sec-q-circ}, there is at least a speed up of $\mathcal{O}(n)$. 

Of-course for quadratic terms  $\{ (t_{ij}, a^\dagger_i a_j) \}$ there is a more efficient way to state the Hamiltonian such that these terms become diagonal. The above argument is to demonstrate the grouping strategies that can be taken in order to take advantage of the quantum circuit in Sec. \ref{sec-q-circ}. 

For higher order terms $\{ (v_{ijkl}, a^\dagger_i a^\dagger_j a_k a_l ) \}$ the situation is more tiresome and is left to the appendix. However, it is shown that at the higher order levels such as $\{ (v_{ijkl}, a^\dagger_i a^\dagger_j a_k a_l ) \}$ a grouping that gives a speed-up of at least 
$\mathcal{O}(n)$ is possible.



 





% %% Index ordering
% For the purpose of the grouping strategy we are about to introduce, it is useful to review the transformation process of second quantized terms in a Hamiltonian onto the Pauli strings. In particular we consider the set of  $\{
% a_i^\dagger a_j^\dagger a_k a_l \}$ that contains all the distinct (normal-ordered) products of two annihilation and two creation operators on $n$ spin-orbital levels of the problem. Every spin-orbital level  becomes equivalent to a qubit in the quantum computer. These qubits are labeled from $1$ to $n$. The total number of terms in the set 
% $\{
% a_i^\dagger a_j^\dagger a_k a_l \}$ is $\binom{n}{2}\binom{n}{2}$ and is of $\mathcal{O}(n^4)$ order. 

% % It is worth to mention that change of sings due to rearranging the operators is always contributes to the corresponding weights of that term. 
% %%%%%

% %%
% By this ordering, from left to right, the first operator acts on the lowest indexed qubit (spin-orbital), the second operator on the second lowest index, etc.
% %%%%
% For example $$\mathcal{I} 
% \left[
% a^\dagger_{2}  a^\dagger_{4}  a_{1} a_{6}\right] 
% =a_{1} a^\dagger_{2} a^\dagger_{4} a_{6}.
% $$


% %%%%%
% Now, consider $\mathcal{I}
% \left[
% a_i^\dagger a_j^\dagger a_k a_l \right]
% $, where no index is repeated. Using the JW transformation in Eqs. (\ref{eq-JW-1}) and (\ref{eq-JW-2}), the final Pauli strings are of the following format:
% \begin{eqnarray}
% \hat{O}_{i_1} 
% \textit{\sout{ $\hat{Z}$ } } 
% \hat{O}_{i_2}
% \textit{\sout{ $\hat{I}$ } }
% \hat{O}_{i_3}
% \textit{\sout{ $\hat{Z}$ } }
% \hat{O}_{i_4},
% \end{eqnarray}
% where 
% \begin{eqnarray}
% \hat{O}_{i} 
% \textit{\sout{ $\hat{Z}$ } } 
% \hat{O}_{j}
% &=& 
% \hat{O}_{i} 
% \otimes
% \left( \bigotimes_{k=i+1}^{k=j-1}\hat{Z}_k \right)
% \otimes
% \hat{O}_{j}
% \end{eqnarray}
% and 
% \begin{eqnarray}
% \hat{O}_{i}
% \textit{\sout{ $\hat{I}$ } }
% \hat{O}_{j}
% &=& 
% \hat{O}_{i} 
% \otimes
% \left( \bigotimes_{k=i+1}^{k=j-1}\hat{I}_k \right)
% \otimes
% \hat{O}_{j}.
% \end{eqnarray}
% Here $\hat{O} \in \{\hat{X}, \hat{Y} \}$. We consider the case where one/two indices is/are repeated, separately.

% In the following we show that we these Pauli strings can be grouped according to the two steps outlined in the previous section.



% % In the case one index is repeated; for example $i_1=i_2$, after JW the Pauli strings are in the form of:
% % \begin{eqnarray}
% % \hat{Z}_{i} 
% % \textit{\sout{ $\hat{I}$ } }
% % \hat{O}_{i_3}
% % \textit{\sout{ $\hat{Z}$ } }
% % \hat{O}_{i_4},
% % \end{eqnarray}





% Following the previous subsection, we would like to group the terms in the Hamiltonian according to the two steps outline above. Once the number of sets $n_g$ is identified and the possibility of step two is guaranteed, the speed-up in the number of measurement is evaluated as $\mathcal{O}(n_h/n_g)$. The grouping strategy we consider is perhaps better illustrated if we just focus on a subset of possible Pauli strings. 

% The factor $2^4$ is a result of JW transformation of a terms such as 
% $a_i^\dagger a_j^\dagger a_k a_l$
% Using the definitions in Eqs. (\ref{eq-JW-1}) and (\ref{eq-JW-2}) in $a_i^\dagger a_j^\dagger a_k a_l$, with no repeated indices, maps it onto a sum of $2^4$ Pauli strings that  are in the form of 



% The total number of Pauli strings from the JW transformation
% of all the $\{
% a_i^\dagger a_j^\dagger a_k a_l \}$ terms in the Hamiltonian is $2^4 \, \binom{n}{4} = \mathcal{O}((2n)^4)$.




==> Archive/grouping_chemistry2.tex <==


% \subsubsection{How to group them}

% A different way to see the $2^4 \, \binom{n}{4}$ Pauli strings is
% as the following: First, let us fix the index of $p_3$ between $[3, n-1]$. For a given fixed $p_3$ there are $\binom{p_3-1}{2}$ ways to choose $p_1$ and $p_2$. Next, consider the values of $p_1$, $p_2$, and $p_3$  as well as the operators of $\hat{O}_1$ $\hat{O}_2$ and $\hat{O}_3$ fixed. Then, define the set $S_{g}$; 
% \begin{eqnarray}
% S_{g} =
% \{\hat{O}_{p_1} 
% \circ \hat{O}_{p_2}
% \circ \hat{O}_{p_3}
% \circ \hat{O}_{p_4} \vert 
% \hat{O}_{p_4} = \hat{X} \textit{  or  } \hat{Y}, 
% \textit{  and  } p_4 >p_3 \}.
% \label{eq-SQ-Sg}
% \end{eqnarray}
% It essentially contains all the strings in which $\hat{O}_{p_4}$ is one of the $\hat{X}$ or $\hat{Y}$ operators, and is applied on any of the qubits between $p_3$ to $n$. At the same time the first three operators and their indices are kept constant and denoted by subscript $g$. Finally, the set of $2^4 \, \binom{n}{4}$ Pauli strings $S_H$ is the union of all $S_g$ groups.  

% In an $S_g$ set defined above, while $p_4$ can be any index greater than $p_3$. For a fixed set of $p_1$, $p_2$, and $p_3$ in the above, and fixed $\hat{O}_{p_1}$, $\hat{O}_{p_2}$, $\hat{O}_{p_3}$, and $\hat{O}_{p_4}$,
% it is easy to verify that all the $(n-p_3)$ Pauli strings anti-commute. The key is that $\hat{O}_{p_4}$ on two strings of this group seats at different indices, and $\hat{X}$($\hat{Y}$) on one string and $\hat{Z}$ on the other string anti-commute. 

% The number of $S_g$ sets, $n_g$,  is counted by noticing that $p_3$ is in  $[3, n-1]$ with two possible Pauli matrix choices for $\hat{O}_3$. For
% every combination, there are  $\binom{p_3}{2} \times 2^2$ different combinations for $\hat{O}_1$ and $\hat{O}_2$. Thus, $n_g$ is of order of:
% \begin{eqnarray}
% n_g &=& 2 \times (2^3  \sum_{p_3=3}^{n-1} \binom{p_3}{2} )  \nonumber \\
%     &=& \mathcal{O} (2^4 n^3) 
% \end{eqnarray}{}
% At the same time the number of total Pauli strings arising from JW mapping of $\{
% a_i^\dagger a_j^\dagger a_k a_l \}$ 
% is $n_h = \mathcal{O}(2^4n^4) $. 

% Before,  we can arrive at the conclusion that the grouping above results in an $\mathcal{O}(n) $ speed-up, we need to show that the step two is also possible; that is we can append a set of auxiliary  Pauli strings such that all the terms in the extended set $M_g$ are mutually anti-commuting, and the number of terms in an extended set $M_g$ 
% is $2^m-1$ for some integer $m$ (this integer may vary for different $M_g$ groups).

% This last step can be done in the following way. First, if $\vert S_g \vert=2^m-1$ for some integer $m$, then step two is already satsfied. If $2^{m-1}-1<\vert S_g \vert<2^m-1$, it is suffice to show that we can increase gradually the elements in the set such that $\vert M_g \vert = 2\times \vert S_g\vert $. The latter ensures we can always  find enough terms to satisfy the condition $\vert M_g \vert = 2^m-1$.

% For a given $S_g$ defined as in Eq. (\ref{eq-SQ-Sg}), define an auxiliary set $A_g$ that is any subset of $S_g$ where the $\hat{O}_4$ is substituted;  If $\hat{O}_4$ is $\hat{X}$ it becomes $\hat{Y}$ and vice versa.
% $A_g$ satisfies the definition Eq. (\ref{eq-aux}). In addition, 


% This approach allows us to increase, up to twice, the number of Pauli strings in a given $S_g$. Thus, The  extended set has $2^m-1$ elements that all anti-commute. Therefore, step two is accomplished.

% Finally we make the conclusion that with the grouping strategy above one can achieve a speed-up in the number of measurements  which is at least linear in the number of qubits of the system; a speed-up of at least  $\mathcal{O}(n)$ with $n$ the number of qubits.


==> Archive/introduction.tex <==
\section{Introduction}
% The approach to the calculation of fermionic quantum chemistry problems on a quantum hardware is based on the mapping of  the Fock space onto qubits, and the second quantized Hamiltonian of the problem onto the languange of Pauli matrices via Jordan Wigner transformation, or other similar transformations.

% In this approach the qubits are initially prepared in a
% quantum state. Upon the sequential action of a series of quantum gates, the quantum circuit, the state of the qubits is brought to a trial wave-function referred to as an ansatz. Since the gates can be parameterized, the ansatz is parametric as well. Thus, running the circuit many times with different paramteters and measuring the Hamiltonian at the end of the circuit at every run, allow to find optimized parameters and the best ansatz that minimizes the energy. Such an algorithm for finding the ground state of a given Hamiltonian 
% that relies on the variational principle is referred to as a Quantum Variational Algorithm. 
% For Quantum Chemistry problems specifically, the quantum circuit is chosen to reflect the physical intuition behind the choice of the ansatz. The ground state of a molecular compound for example is physically thought to be a superposition sum of a set of Fock bases. Such a basis must be, physically, an excitation above a reference unperturbed initial state such as a Hartree-Fock. Thus a quantum circuit that attempts to generate a superposition of a set of single, double, and higher excitaions above a reference state is mostly demanded. A theoretical well understood and accepted example is the  Unitary Coupled Cluster approach. The UCC in practice is approximated via Trotterization and perhaps other phenomenological reasoning in order to be practically implementable on a quantum hardware.



% %%% challenges and computational cost of UCC
% While VQA approach to Hybrid quantum-classical computation has shown astonishing success both at theory and Hardware (IBM, Nature adapt), the computational cost of this method can be overwhelmingly high. In particular, the implementation of the UCC in terms of parametric one-qubit and two-qubit gates requires break-down of many-qubit gates implied in UCC ansatz. This decomposition increases the depth of the quantum circuit which is already polynomial function of the number of qubits; For example the UCCSD ansatz that only takes into account the single and double excitations can have up-to $\mathcal{O}(N^4)$ terms, which translate to the same and even higher quantum circuit depth. 

% In addition, optimization of parameters requires of running the circuit thousands of times in order to be able to update the paprameters as part of the optimization. The optimization relies on classical optimizer that makes and already noisy quantum calculation   exposed to an additional classical optimization problem.

% There are different scheme in reducing the number of qubits in a problem (Bravey), performing post- and pre-processing (reducing qubits Babush active space), and other alternative parametric ansatz (entangler). nevertheless, a fundamental solution to the limitations of NISQ device coherence time is not garantueed generally.  

% In this paper we propose a different route for finding the ground state and energy of a given interacting many-body electronic system. In contrast to VQA,  there is no parameter or optimization in our proposed method. We use the quantum processor to measure the Hamiltonian with respect to different rotated basis. The rotational of the basis are done by using an additional set of qubits - the  ancillary qubits -  in addition to the qubits representing the simulated problem  which we refer to as the physical qubits. Through the design of the quantum circuit, the ancillary qubits are entangled to the physical qubits that allows the measuremnt of the Hamiltonian in different basis sets. The latter can be seen as interference of different wave-fuctions as explained in ref (goog prl), which uses interference to evaluate off-diagonal elements.

% The number of measurements are kept as a polynomial function of number of qubits. Next, using the result of the measurements and by post-processing on a classical computer, an EHM is constructed. The dimension of the latter is kept limited such that the EHM can be diagonalized on a classical computer. Upon diagonalization of the effective Hamiltonian, the ground state and some low-lying excited states of the system are found.

% A strong advantage of our approach in comparison to 
% VQA is the absence of parameters and optimization and provides advantage in terms of time-complexity of the computation. Secondly, the depth of the quantum circuit can be controlled; the diagonal matrix elements in EHM can be calculated with no circuit depth, the off-diagonal elements can be evaluted by change of basis on the ancillary qubits as first noted in (GOOG PRL). the latter depending on the row and column of the element may require higher quantum circuit depth. The maximum depth never exceeds the depth implied in UCC ansatz. The overall shorter depth makes our approach suited for NISQ low coherence times. In terms of measurements, our approach measures the Hamiltonian in the same way that is done with VQAs; that is measurement of each individual term in a given Hamiltonian. 














==> Figures/Figure-CoreCircuit.tex <==
%% Figure corresponding to the different circuits

\captionsetup[subfigure]{position=top, labelfont=bf,textfont=normalfont,justification=raggedright,format=plain}
\begin{subfigure}{0.45\textwidth}
  \caption{}
  \begin{quantikz}
        \lstick{$\ket{0}$}  
        &\gate{H}
        &\octrl{1}\qw
        &\ctrl{1}
        & \gate{H}
        & \qw
        \\
        \lstick{$\ket{0}^{\otimes N}$} 
        &\qwbundle[alternate]{}
        & \gate{n^\prime} \qwbundle[alternate]{} 
        & \gate{n} \qwbundle[alternate]{} 
        & \qwbundle[alternate]{}
        & \qwbundle[alternate]{}
        \end{quantikz} 
  \label{subfig:sub1:fig:core-circ}
\end{subfigure}

\vspace{1cm}

\begin{subfigure}{0.45\textwidth}
  \caption{}
  \begin{quantikz}
        \lstick{$\ket{0}$}  
        &\gate{H}
        &\octrl{1}\qw
        &\ctrl{1}\qw
        & \gate{S}
        & \gate{H}
        &\qw
        \\
        \lstick{$\ket{0}^{\otimes N}$} 
        &\qwbundle[alternate]{}
        & \gate{n^\prime} \qwbundle[alternate]{} 
        & \gate{n} \qwbundle[alternate]{} 
        & \qwbundle[alternate]{}
        & \qwbundle[alternate]{}
        & \qwbundle[alternate]{}
        \end{quantikz} 
  \label{subfig:sub2:fig:core-circ}
\end{subfigure}

\vspace{1 cm}

\begin{subfigure}{0.45\textwidth}
  \caption{}
  \begin{quantikz}
        \lstick{$\ket{0}$}  
        &\ctrl{1}\qw
        &\qw
        \\
        \lstick{$\ket{0}^{\otimes 3}$} 
        & \gate{n} \qwbundle[alternate]{} 
        & \qwbundle[alternate]{} 
        \end{quantikz}  $\rightarrow$
        \begin{quantikz}
        \lstick{$\ket{0}$}  
        &\ctrl{1}\qw
        &\ctrl{2}\qw
        & \qw
        \\
        \lstick{$\ket{0}$} 
        &\gate{X} \qw
        & \qw
        & \qw
        \\
        \lstick{$\ket{0}$} 
        &\qw
        &\gate{X} \qw
        & \qw
        \\
        \lstick{$\ket{0}$} 
        &\qw
        &\qw
        &\qw
        \end{quantikz} 
  \label{subfig:sub3:fig:core-cirq}
\end{subfigure}

==> Figures/circuit1.tex <==
% \begin{figure*}
% \begin{subfigure}{.325\textwidth}
% %   \centering
%   \caption{}
%   \begin{quantikz}
%         \lstick{$\ket{0}$}  
%         &\gate{H}
%         &\octrl{1}\qw
%         &\ctrl{1}
%         & \gate{H}
%         \\
%         \lstick{$\ket{0}^{\otimes N}$} 
%         &\qwbundle[alternate]{}
%         & \gate{\hat{n}} \qwbundle[alternate]{} 
%         & \gate{\hat{n}^\prime} \qwbundle[alternate]{} 
%         & \qwbundle[alternate]{}
%         \end{quantikz} 
%   \label{fig:sub2}
% \end{subfigure}
% %
% %
% %
% \begin{subfigure}{.35\textwidth}
% %   \centering
%   \caption{}
%   \begin{quantikz}
%         \lstick{$\ket{0}$}  
%         &\gate{H}
%         &\octrl{1}\qw
%         &\ctrl{1}\qw
%         & \gate{S}
%         & \gate{H}
%         \\
%         \lstick{$\ket{0}^{\otimes N}$} 
%         &\qwbundle[alternate]{}
%         & \gate{\hat{n}} \qwbundle[alternate]{} 
%         & \gate{\hat{n}^\prime} \qwbundle[alternate]{} 
%         & \qwbundle[alternate]{}
%         & \qwbundle[alternate]{}
%         \end{quantikz} 
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Quantum circuits designed to measuring the off-diagonal elements 
% of a effective Hamiltonian with only two basis $\ket{\bf n^\prime}$ and $\ket{\bf n}$. (a)  circuit to measure the real part of the off-diagonal element (b) circuit to measure the imaginary part of the off-diagonal element.}
% \label{fig:core-circ}
% \end{figure*}





